Time-uniform central limit theory and asymptotic confidence sequences

Confidence intervals based on the central limit theorem (CLT) are a cornerstone of classical statistics. Despite being only asymptotically valid, they are ubiquitous because they permit statistical inference under weak assumptions and can often be applied to problems even when nonasymptotic inference is impossible. This paper introduces time-uniform analogues of such asymptotic confidence intervals, adding to the literature on confidence sequences (CS) -- sequences of confidence intervals that are uniformly valid over time -- which provide valid inference at arbitrary stopping times and incur no penalties for "peeking" at the data, unlike classical confidence intervals which require the sample size to be fixed in advance. Existing CSs in the literature are nonasymptotic, enjoying finite-sample guarantees but not the aforementioned broad applicability of asymptotic confidence intervals. This work provides a definition for "asymptotic CSs" and a general recipe for deriving them. Asymptotic CSs forgo nonasymptotic validity for CLT-like versatility and (asymptotic) time-uniform guarantees. While the CLT approximates the distribution of a sample average by that of a Gaussian for a fixed sample size, we use strong invariance principles (stemming from the seminal 1960s work of Strassen) to uniformly approximate the entire sample average process by an implicit Gaussian process. As an illustration, we derive asymptotic CSs for the average treatment effect in observational studies (for which nonasymptotic bounds are essentially impossible to derive even in the fixed-time regime) as well as randomized experiments, enabling causal inference in sequential environments.

==> simulation_details.tex <==
\section{Simulation details}
\subsection{Simulated randomized experiment (\cref{fig:CS_randomized})}
\label{section:simulationRandomized}
First, we describe the simulated randomized sequential experiment displayed in \cref{fig:CS_randomized}.
\paragraph*{Data-generating process} Consider a randomized experiment with $n = 10^4$ subjects, each with 3 real-valued covariates. Generate $10^4$ 3-tuples of said covariates $X_1, X_2, \dots \simiid N_3(0, I_3)$ from a standard trivariate Gaussian.
Randomly assign subjects to treatment or control groups with equal probability: $A_1, \dots, A_n \sim \text{Bernoulli}(1/2)$. Define the regression function,
\begin{equation}
\label{eq:simulationRegressionFunction}
    \mu^\star(x_i) := 1 - x_{i, 1}^2 - 2\sin(x_{i,2}) + 3|x_{i, 3}|,
\end{equation}
and the target parameter $\psi := 1$ (which we will ensure is the average treatment effect by design).
Finally, generate outcomes $Y_1, \dots, Y_n$ as
\[ Y_i := \mu^\star(X_{i, 1}, X_{i, 2}, X_{i,3}) + \psi\cdot A_i + \epsilon_i,
\]
where $\epsilon_i \simiid t_{5}$ are drawn from a $t$-distribution with 5 degrees of freedom (we use this heavy-tailed distribution in an attempt to stress-test the finite fourth absolute moment condition of Theorems~\ref{theorem:csate_randomized} and \ref{theorem:csate_observational}). We now describe the three models used to estimate $\psi$ knowing the treatment assignment distribution of $A_1, \dots, A_n$ but without knowledge of $\mu^\star$ or the distribution of $\epsilon_i$.

\paragraph*{Estimators}
The IPW estimator $\widehat \psi_t^\mathrm{IPW}$ used in this example is the simplest of the three and takes the form,
\begin{equation}
\label{eq:unadjustedEstimator}
    \widehat \psi_t^\mathrm{IPW} := \frac{1}{t} \sum_{i=1}^t \left ( \frac{A_i}{1/2} - \frac{1-A_i}{1/2} \right ) Y_i.
\end{equation}
Since this estimator does not estimate the regression functions $\mu^a$ for $a = 0, 1$, no sequential cross-fitting is needed.
The other two estimators employ sequential cross-fitting as in \cref{section:seqSampleSplit} and take the form \eqref{eq:cross_fit_estimator} but with various choices of $\widehat \mu_t^1$ and $\widehat \mu_t^0$. Specifically, the \emph{parametric} AIPW estimator uses linear regression to construct $\widehat \mu_t^1$ and $\widehat \mu_t^0$ which in this case is misspecified. The stacking-based AIPW estimator uses a weighted ensemble of several machine learning algorithms. In this simulation, these consisted of adaptive regression splines, generalized additive models, generalized linear models with LASSO ($\ell_1$ regularization) and pairwise interactions, and random forests. The weights were chosen via cross-validation \citep{van2007super,polley2011super}. We then applied Theorem~\ref{theorem:csate_randomized} to obtain the confidence sequences displayed in \cref{fig:CS_randomized}.

\subsection{Simulated observational study (\cref{fig:CS_observational})}
\label{section:simulationObservational}

\paragraph*{Data-generating process} The simulation scenario used to produce~\cref{fig:CS_observational} is identical to the previous section but without complete Bernoulli randomization of treatments. Instead, each individual is assigned treatment with propensity score $\pi(x_1, x_2, x_3)$, defined by
\[ \pi(x_1, x_2, x_3) := 0.2 + 0.6\cdot \logit \left ( \mu^\star(x_1, x_2, x_3) \right ), \]
where $\mu^\star$ is the regression function defined in \eqref{eq:simulationRegressionFunction}. A scale of 0.6 and a translation of 0.2 is applied to ensure that $\pi(x_1, x_2, x_3) \in [0.2, 0.8]$ is bounded away from 0 and 1.

\paragraph*{Estimators}
Here, we use a difference-in-means estimator\footnote{While the form given in \eqref{eq:difference-in-means-estimator} may not visually resemble the typical difference in means estimator, it is easy to check that for any fixed $t$, they are equivalent. We only write it in the given form to make compatibility with \asympcs{}s more transparent.} given by
\begin{equation}\label{eq:difference-in-means-estimator}
  \widehat \psi_t^\mathrm{DIM} := \frac{1}{t} \sum_{i=1}^t \left ( \frac{A_i}{\frac{1}{t}\sum_{j=1}^t A_j} - \frac{1-A_i}{1-\frac{1}{t}\sum_{j=1}^t A_j}  \right ) Y_i
\end{equation}
which does not make use of sequential cross-fitting. On the other hand, the parametric and stacking-based AIPW estimators invoke sequential cross-fitting and take the form \eqref{eq:cross_fit_estimator} where $\widehat \mu_t^a$ is constructed in the same way as in the experimental setup of the previous section but since $\pi(x)$ is unknown, it must now be estimated. The parametric AIPW estimator uses logistic regression to accomplish this, while the stacked ensemble is the same as that used for regression (but with appropriate modifications made for classification). Invoking Theorem~\ref{theorem:csate_observational} yields the \asympcs{}s of~\cref{fig:CS_observational}.

\subsection{Width and coverage simulations}

Here, we briefly describe the simulation setup used to produce the plots in \cref{section:simulations-width-coverage}. Applications of \asympcs{}s follow straightforwardly from \namecref{theorem:acs}s~\ref{theorem:acs} and~\ref{theorem:csate_randomized} (and analogously for fixed-time CLT-based \ci{}s).
We displayed these alongside the sub-Gaussian \cs{} of \citet{robbins1970statistical} (see also \citep[\S 3.2]{howard2018uniform}) and the sub-exponential \cs{} of \citet[Thm 4 and Cor 2]{howard2018uniform}, both of which are nonasymptotic. These nonasymptotic \cs{}s are immediately applicable to the settings considered in \cref{section:simulations-width-coverage} since the observations (or influence functions in the context of causal inference) are themselves bounded and hence sub-Gaussian (and hence sub-exponential). The data for these simulations were generated as follows.

\begin{enumerate}[label = (\alph*)]
\item \textbf{Estimating the mean of bounded random variables.}

  \noindent As mentioned in \cref{fig:widths_miscoverage}, observations were generated as $\infseqt{Y_t} \sim \mathrm{Unif}[0, 1]$. The boundedness of these random variables implies that they are $\sigma$-sub-Gaussian with $\sigma = 1/2$ and sub-$\psi$ with an empirical ``variance process'' and $\psi$ being the cumulant generating function (CGF) of an exponential distribution.\footnote{The notion of ``sub-$\psi$'' used throughout \citet{howard2018uniform} is slightly different than what one might think of when they hear ``sub-exponential'' since the authors do not necessarily require upper-bounding of the CGF of the random variables themselves, but instead require that when the CGF is subtracted off and pre-multiplied by a ``variance process'', the exponential Chernoff process is conditionally upper-bounded by one (which is a weaker requirement than upper-bounding the CGF). For more details see \citet{howard2018uniform}.} Importantly for our purposes, the sub-Gaussian and sub-exponential \cs{}s of their paper are immediately applicable.
  
\item \textbf{Estimating the ATE in a completely randomized Bernoulli experiment:}

  \noindent 
  
\item \textbf{Estimating the ATE in an experiment with personalized randomization:}
\end{enumerate}
\TODO{finish}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_aos"
%%% End:

